All You May Need for VQA are Image Captions

Visual Question Answering (VQA) has benefited from increasingly sophisticated models, but has not enjoyed the same level of engagement in terms of data creation. In this paper, we propose a method that automatically derives VQA examples at volume, by leveraging the abundance of existing image-caption annotations combined with neural models for textual question generation. We show that the resulting data is of high-quality. VQA models trained on our data improve state-of-the-art zero-shot accuracy by double digits and achieve a level of robustness that lacks in the same model trained on human-annotated VQA data.

==> data_analysis.tex <==
%auto-ignore

\begin{table*}[t]
\centering
\small		
\begin{tabular}{|l|c|c|c|l|}
\hline
Question Prefix &  \vqaset \% & \qsqcoco \% & \qsqcc \% & Question Example from \qsqcoco\\
\hline
        \qex{What is} &       0.140 &             0.288 &             0.217 &                       \qex{What is the man swinging?} \\
         \qex{Is the} &       0.098 &             0.084 &             0.053 &                \qex{Is the baby wearing a Santa hat?} \\
      \qex{What kind} &       0.025 &             0.049 &             0.078 &           \qex{What kind of truck is the yellow one?} \\
       \qex{How many} &       0.110 &             0.022 &             0.005 &  \qex{How many people are standing in front of a tv?} \\
     \qex{What color} &       0.090 &             0.022 &             0.018 &                   \qex{What color is the man's hair?} \\
       \qex{Where is} &       0.019 &             0.071 &             0.034 &            \qex{Where is the tennis player pictured?} \\
        \qex{Is this} &       0.082 &             0.008 &             0.015 &                      \qex{Is this a safe way to fly?} \\
       \qex{What are} &       0.024 &             0.049 &             0.022 &   \qex{What are the sheep and other animals roaming?} \\
         \qex{Who is} &       0.005 &             0.054 &             0.020 &                            \qex{Who is in the photo?} \\
       \qex{Is there} &       0.037 &             0.011 &             0.022 &                \qex{Is there a pool in the backyard?} \\
      \qex{What does} &       0.011 &             0.015 &             0.038 &      \qex{What does a giraffe do with its long neck?} \\
        \qex{Are the} &       0.024 &             0.022 &             0.007 &      \qex{Are the apples on the cutting board green?} \\
      \qex{Where are} &       0.006 &             0.032 &             0.014 &       \qex{Where are the skateboarders in the photo?} \\
      \qex{What type} &       0.018 &             0.006 &             0.022 &                   \qex{What type of picture is this?} \\
       \qex{What was} &       0.000 &             0.009 &             0.023 &                  \qex{What was the woman looking at?} \\
       \qex{Does the} &       0.014 &             0.007 &             0.007 &          \qex{Does the adult giraffe have any young?} \\
      \qex{Are there} &       0.020 &             0.002 &             0.004 &          \qex{Are there any exceptions to this rule?} \\
        \qex{What do} &       0.002 &             0.003 &             0.018 &                \qex{What do the father and son ride?} \\
       \qex{What did} &       0.000 &             0.001 &             0.021 &                 \qex{What did the cat lay inside of?} \\
          \qex{Is it} &       0.017 &             0.001 &             0.005 &            \qex{Is it possible to eat a whole pizza?} \\
\hline
\end{tabular}
\caption{Most popular question prefix distribution on valid questions whose answers are in the 6k target vocabulary.}
\label{tab:coco_prefix_stats}
\end{table*}

\section{Analysis of Generated Data}
\label{sec:data_analysis}

Table~\ref{tab:coco_prefix_stats} presents the top question prefixes and their distribution in the \vqaset and \qsq-based dev sets, showing significant differences between datasets. Many questions in \vqaset are of boolean answer type, e.g. \qex{is the}, \qex{is there} and \qex{does the}, summing to 36.9\%. In addition, (\qex{how many}) questions are frequent, 11\%. Finally, questions for the color attribute are standing out with 9.2\%. 
On the other hand, \coco and \ccslong questions are more explanatory in nature, with the majority of questions (more than 50\%) of the form \qex{what is/are/do/does/type}. Another type that is more prominent in \coco and \ccslong are \qex{where is} questions, which are at least twice or more frequent compared to \vqaset.
More analysis is in Appendix~\ref{apdx:data_analysis}.

